MODOC: A Modular Interface for Flexible Interlinking of Text Retrieval and Text Generation Functions

Large Language Models (LLMs) produce eloquent texts but often the content they generate needs to be verified. Traditional information retrieval systems can assist with this task, but most systems have not been designed with LLM-generated queries in mind. As such, there is a compelling need for integrated systems that provide both retrieval and generation functionality within a single user interface. We present MODOC, a modular user interface that leverages the capabilities of LLMs and provides assistance with detecting their confabulations, promoting integrity in scientific writing. MODOC represents a significant step forward in scientific writing assistance. Its modular architecture supports flexible functions for retrieving information and for writing and generating text in a single, user-friendly interface.

==> figures/read-module-target-list.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\textwidth]{./figures/read-module-target-list-file.png}
    \caption{This view presents a comprehensive list of all text aligned using the selected text from the source document as input for the text alignment retrieval function.}
    \label{fig:read-module-target-list}
\end{figure*}


